A Hilbert space approach to effective resistance metric

A resistance network is a connected graph $(G,c)$. The conductance function $c_{xy}$ weights the edges, which are then interpreted as conductors of possibly varying strengths. The Dirichlet energy form $\mathcal E$ produces a Hilbert space structure (which we call the energy space ${\mathcal H}_{\mathcal E}$) on the space of functions of finite energy. We use the reproducing kernel $\{v_x\}$ constructed in \cite{DGG} to analyze the effective resistance $R$, which is a natural metric for such a network. It is known that when $(G,c)$ supports nonconstant harmonic functions of finite energy, the effective resistance metric is not unique. The two most natural choices for $R(x,y)$ are the ``free resistance'' $R^F$, and the ``wired resistance'' $R^W$. We define $R^F$ and $R^W$ in terms of the functions $v_x$ (and certain projections of them). This provides a way to express $R^F$ and $R^W$ as norms of certain operators, and explain $R^F \neq R^W$ in terms of Neumann vs. Dirichlet boundary conditions. We show that the metric space $(G,R^F)$ embeds isometrically into ${\mathcal H}_{\mathcal E}$, and the metric space $(G,R^W)$ embeds isometrically into the closure of the space of finitely supported functions; a subspace of ${\mathcal H}_{\mathcal E}$. Typically, $R^F$ and $R^W$ are computed as limits of restrictions to finite subnetworks. A third formulation $R^{tr}$ is given in terms of the trace of the Dirichlet form $\mathcal E$ to finite subnetworks. A probabilistic approach shows that in the limit, $R^{tr}$ coincides with $R^F$. This suggests a comparison between the probabilistic interpretations of $R^F$ vs. $R^W$.

==> finite-networks.tex <==
%%!TEX root = ERM.tex

\section{Effective resistance}
\label{sec:Effective-resistance}

\subsection{Resistance metric on finite networks}
\label{sec:Resistance-metric-on-finite-networks}

We make the standing assumption that the network is finite in \S\ref{sec:Resistance-metric-on-finite-networks}. However, the results actually remain true on any network for which $\Harm = 0$.

\begin{defn}\label{def:effective-resistance}
  If one amp of current is inserted into the \ERN at $x$ and withdrawn at $y$, then the \emph{(effective) resistance} $R(x,y)$ is the voltage drop between the vertices $x$ and $y$.
  \glossary{name={$R$},description={resistance metric},sort=r,format=textbf}
\end{defn}

\begin{theorem}\label{thm:effective-resistance-metric}
  The resistance $R(x,y)$ has the following equivalent formulations:
  \linenopax
  \begin{align}
    R(x,y)
    &= \{v(x)-v(y) \suth \Lap v = \gd_x-\gd_y\}
    \label{eqn:def:R(x,y)-Lap} \\
    &= \{\energy(v) \suth \Lap v = \gd_x-\gd_y\} \label{eqn:def:R(x,y)-energy} \\
    &= \min \{\diss(\curr) \suth \curr \in \Flo(x,y)\} \label{eqn:def:R(x,y)-diss} \\
    &= 1/\min \{\energy(v) \suth v(x)=1, v(y)=0, v \in \dom\energy\} \label{eqn:def:R(x,y)-R} \\
    &= \min \{\gk \geq 0 \suth |v(x)-v(y)|^2 \leq \gk \energy(v), v \in \dom\energy\} \label{eqn:def:R(x,y)-S} \\
    &= \sup \{|v(x)-v(y)|^2 \suth \energy(v) \leq 1, v \in \dom\energy\} \label{eqn:def:R(x,y)-sup}.
  \end{align}
\end{theorem}

We leave the proof of Theorem~\ref{thm:effective-resistance-metric} as an exercise; we suggest using the energy kernel to take several shortcuts. A complete proof appears in \cite[Thm.~5.2]{OTERN} and patches some holes in the literature. The authors first learned of the effective resistance metric from \cite{Pow76b}) and \cite{Kig01,Str06}, respectively; we have not seen \eqref{eqn:def:R(x,y)-energy} or \eqref{eqn:def:R(x,y)-sup} in the literature previously. It is clear that \eqref{eqn:def:R(x,y)-sup} is equivalent to \eqref{eqn:def:R(x,y)-S} by considering the norm of the operator $L_{xy}$ defined by $L_{xy} u := u(x) - u(y)$. In fact, $L_{xy} = L_x - L_y$, where the evaluation operators $L_x$ are used in the definition of $v_x$ in \cite{DGG}, and this is how we were led to \eqref{eqn:def:R(x,y)-sup}. Taking the minimum (rather than the infimum) in \eqref{eqn:def:R(x,y)-diss}, etc, is justified because a quadratic form always attains its minimum on a closed convex set.

\begin{remark}[Resistance distance via network reduction]
  \label{rem:Resistance-distance-via-network-reduction}
  Let $H$ be a (connected) planar subnetwork of a finite network $G$ and pick any $x,y \in H$. Then $H$ may be reduced to a trivial network consisting only of these two vertices and a single edge between them via the use of three basic transformations: (i) series reduction, (ii) parallel reduction, and (iii) the $\nabla$-\textsf{Y} transform \cite{Epifanov66,Truemper89}. Each of these transformations preserves the resistance properties of the subnetwork, that is, for $x,y \in G \less H$, $R(x,y)$ remains unchanged when these transformations are applied to $H$. The effective resistance between $x$ and $y$ may be interpreted as the resistance of the resulting single edge. An elementary example is shown in Figure~\ref{fig:network-reduction}. A more sophisticated technique of network reduction is given by the trace (Schur complement) construction of Remark~\ref{rem:Resistance-distance-via-Schur-complement}.
\end{remark}

  \begin{figure}%[h]
    \centering
    \includegraphics{network-reduction.eps}
    \caption{\captionsize Effective resistance as network reduction to a trivial network. This basic example uses parallel reduction followed by series reduction; see Remark~\ref{rem:Resistance-distance-via-network-reduction}.}
    \label{fig:network-reduction}
  \end{figure}

The following result is not new (see, e.g. \cite[\S2.3]{Kig01}), but the proof given here is substantially simpler than most others found in the literature.

\begin{lemma}\label{thm:R-is-a-metric}
  $R$ is a metric.
  \begin{proof}
    Symmetry and positive definiteness are immediate from \eqref{eqn:def:R(x,y)-energy}, we use \eqref{eqn:def:R(x,y)-Lap} and the energy kernel to check the triangle inequality. Let $v_1 = v_x - v_y$, $v_2 = v_y - v_z$, and $v_3 := v_1 + v_2$.
    % satisfies $\Lap v_3 = \gd_x - \gd_z$. 
    %For $s \nbr t$, it is clear that $v_3(s)-v_3(t) = v_1(s) - v_1(t) + v_2(s) - v_2(t)$. By summing along any path from $x$ to $z$, one sees that this remains true for $s \notnbr t$, whence
    \linenopax
    \begin{align*}
      R(x,z)
      = v_3(x)-v_3(z)
      &= v_1(x)-v_1(z) + v_2(x)-v_2(z) \\
      &\leq v_1(x)-v_1(y) + v_2(y)-v_2(z)
      %= v_1(x)-v_1(y) + v_2(y)-v_2(z)
      = R(x,y) + R(y,z),
    \end{align*}
    because $y$ is the minimum of $v_1$ and the maximum of $v_2$. This follows from the minimum principle for harmonic functions on the finite set $\verts\less\{y\}$ and the definition of \Lap. See \cite[\S2.1]{Lyons:ProbOnTrees}, for example, or \cite{LevPerWil08}.
  \end{proof}
\end{lemma}

